Combination of CDF and D0 W-Boson Mass Measurements

We summarize and combine direct measurements of the mass of the $W$ boson in $\sqrt{s} = 1.96 \text{TeV}$ proton-antiproton collision data collected by CDF and D0 experiments at the Fermilab Tevatron Collider. Earlier measurements from CDF and D0 are combined with the two latest, more precise measurements: a CDF measurement in the electron and muon channels using data corresponding to $2.2 \mathrm{fb}^{-1}$ of integrated luminosity, and a D0 measurement in the electron channel using data corresponding to $4.3 \mathrm{fb}^{-1}$ of integrated luminosity. The resulting Tevatron average for the mass of the $W$ boson is $\MW = 80\,387 \pm 16 \text{MeV}$. Including measurements obtained in electron-positron collisions at LEP yields the most precise value of $\MW = 80\,385 \pm 15 \text{MeV}$.

==> acknowledgement.tex <==
% acknowledgement.tex                            11 July 2013 (CDF+D0)
%
We thank the Fermilab staff and the technical staffs of the participating institutions for their vital contributions
and acknowledge support from the
DOE and NSF (USA);
ARC (Australia);
CNPq, FAPERJ, FAPESP, and FUNDUNESP (Brazil);
NSERC (Canada);
CAS and CNSF (China);
Colciencias (Colombia);
MSMT and GACR (Czech Republic);
the Academy of Finland;
CEA and CNRS/IN2P3 (France);
BMBF and DFG (Germany);
DAE and DST (India);
SFI (Ireland);
INFN (Italy);
MEXT (Japan);
the Korean World Class University Program and NRF (Korea);
CONACyT (Mexico);
FOM (The Netherlands);
MON, NRC KI, and RFBR (Russia);
the Slovak R\&D Agency (Slovakia);
the Ministerio de Ciencia e Innovaci\'{o}n, and Programa Consolider-Ingenio 2010 (Spain);
the Swedish Research Council (Sweden);
SNSF (Switzerland);
STFC and the Royal Society (United Kingdom);
and the A. P. Sloan Foundation (USA).

%


==> thebib.tex <==
\label{sec:thebib}

\begin{thebibliography}{99} 

\bibitem{lhc-higgs}  
 G. Aad \emph{et~al.} (ATLAS Collaboration), Phys. Lett. B \textbf{716} (2012);  
 S. Chatrchyan \emph{et~al.} (CMS Collaboration), Phys. Lett. B \textbf{716} (2012).

\bibitem{ashujan}
A. V. Kotwal and J. Stark, Ann. Rev. Nucl. Part. Sci. {\bf 58}, 147 (2008).

\bibitem{TEV09} 
CDF and D0 Collaborations, and Tevatron Electroweak Working Group, arXiv:0908.1374 [hep-ex] (2009).

\bibitem{Units}
We use units where $c=1$ throughout this article.

\bibitem{top}
T. Aaltonen \emph{et al.} (CDF and {D0} Collaborations), Phys. Rev. D \textbf{86}, 092003 (2012).


\bibitem{cor-rad}
M. Awramik  \emph{et al.}, Phys. Rev. D \textbf{69}, 053006 (2004).

\bibitem{Wwidth}
CDF and D0 Collaborations, and Tevatron Electroweak Working Group, arXiv:1003.2826 [hep-ex] (2010).

\bibitem{MW-CDF-RunZ}
F.~Abe \emph{et~al.} (CDF Collaboration),  
Phys. Rev. D \textbf{43}, 2070 (1991).

\bibitem{MW-CDF-RUN1A}
F.~Abe \emph{et~al.} (CDF Collaboration),    
Phys. Rev. D \textbf{52}, 4784 (1995).

\bibitem{MW-CDF-RUN1B}
T. Affolder \emph{et~al.} (CDF Collaboration),   
Phys. Rev. D \textbf{64}, 052001 (2001).

\bibitem{MW-CDF-RUN2a}
T.~Aaltonen \emph{et~al.} (CDF Collaboration),   
Phys. Rev. Lett. \textbf{99}, 151801 (2007); Phys. Rev. D \textbf{77}, 112001 (2008).

\bibitem{MW-D0-Ia} 

S. Abachi \emph{et al.} ({D0} Collaboration), Phys. Rev. Lett. \textbf{77}, 3309 (1996).

\bibitem{MW-D0-I}
B.~Abbott \emph{et~al.} ({D0} Collaboration),  
Phys. Rev. D \textbf{58},  012002 (1998).

\bibitem{MW-D0-I-rap}
B.~Abbott \emph{et~al.} ({D0} Collaboration),   
Phys. Rev. D \textbf{62}, 092006 (2000).

\bibitem{MW-D0-I-edge}
V.M.~Abazov \emph{et~al.} ({D0} Collaboration),   
Phys. Rev. D \textbf{66}, 012001 (2002).

\bibitem{MW-D0-RUN2a}
V.M.~Abazov \emph{et~al.} ({D0} Collaboration), 
Phys. Rev. Lett. \textbf{103}, 141801 (2009).

\bibitem{MW-CDF-RUN2}
T.~Aaltonen \emph{et al.} (CDF Collaboration),  
  Phys. Rev. Lett. \textbf{108}, 151803 (2012).
 

\bibitem{MW-D0-Run2b}
V.M.~Abazov \emph{et~al.} ({D0} Collaboration), 
 Phys. Rev. Lett. \textbf{108}, 151804, (2012).


\bibitem{TEV08} 
CDF and D0 Collaborations, and Tevatron Electroweak Working Group, arXiv:0808.0147 [hep-ex] (2008).


\bibitem{MWGW-RunI-PRD}
 V.M.~Abazov \emph{et~al.} (CDF and {D0} Collaborations),       
Phys. Rev. D \textbf{70}, 092008 (2004).

\bibitem{BLUE}
L.~Lyons, D.~Gibaut, and P.~Clifford, 
Nucl. Instrum. Methods Phys. Res., Sect. A, \textbf{270}, 110 (1988);  
A.~Valassi,  Nucl. Instrum. Methods Phys. Res., Sect. A, \textbf{500}, 391 (2003).



\bibitem{cdf_det}
T.~Aaltonen \emph{et al.} (CDF Collaboration), Phys. Rev. D \textbf{77}, 112001 (2008).
 
%\bibitem{d0_det}
%{D0} Collaboration, S.~Abachi \emph{et~al.},
% Nucl. Instrum. and Methods  \textbf{A338}, 185 (1994). 
 
 \bibitem{d0_det}
 V.~M.~Abazov \emph{et~al.} ({D0} Collaboration),  
 Nucl. Instrum. Methods  Phys. Res., Sect. A, \textbf{565}, 463 (2006). 

\bibitem{Etmiss}
$\METl = -(\vec{p}_T^{\ell} + \vec{u}_T)$ where $\vec{u}_T$ is the vector sum of calorimetric $\vec{p}_T$ excluding the charged lepton(s).   

\bibitem{resbos}
C. Bal\'{a}zs and C.P. Yuan, Phys. Rev. D \textbf{56}, 5558 (1997).

\bibitem{blny}
F. Landry \emph{et~al.}, Phys. Rev. D \textbf{67}, 073016 (2003).

\bibitem{cteq66} P. Nadolsky \emph {et~al.}, 
Phys. Rev. D \textbf{78}, 013004 (2008).

\bibitem{ref:PHOTOS}  P. Golonka and Z. Was,  
Eur. J. Phys. C \textbf{45}, 97 (2006).

\bibitem{lep}  
ALEPH, DELPHI, L3 and OPAL, and SLD Collaborations, and LEP Electroweak Working Group, SLD Electrowe\ 
ak and Heavy Flavor Groups, S.~Schael \emph {et~al}, Phys. Rept. B \textbf{427}, 257 (2006);   
ALEPH, DELPHI, L3, OPAL Collaborations, and LEP Electroweak Working Group, arXiv:1302.3415 [hep-ex] \ 
(2013), submitted to Physics Reports. 

\bibitem{geant}
R. Brun and F. Carminati, CERN Program Library Long Writeup \textbf{W5013} (1993).

%\bibitem{pdgwidth}Eq. 43.57 in The Review of Particle Physics. J. Beringer et al. (Particle Data Group), Phys. Rev. D86, 010001 (2012)

\bibitem{PR}
P.~Renton, arXiv:0804.4779 [hep-ex] (2008) and private communications.

\bibitem{cdf-d0-wmass2012}
CDF and D0 Collaborations, and Tevatron Electroweak Working Group, arXiv:1204.0042 [hep-ex] (2012).

\bibitem{CTEQ61M}
  D.~Stump, J.~Huston, J.~Pumplin, W.~K.~Tung, H.~L.~Lai, S.~Kuhlmann, and J.~F.~Owens, 
  J. High Energy Phys. 10, 46 (2003).

\bibitem{mstw2008} A. D. Martin, W. J. Stirling, R. S. Thorne, and
  G. Watt,
Eur. Phys. J. C \textbf{63}, 189 (2009).


\bibitem{ref:WGRAD}
  U.~Baur, S.~Keller, and D.~Wackeroth,
  Phys.\ Rev.\  D \textbf {59}, 013002 (1999).

\bibitem{horace}
C.M. Carloni Calame, G. Montagna, O. Nicrosini, and A. Vicini, 
J. High Energy Phys. 109,10 (2007). 


\bibitem{gfitter}
M. Baak \textit{et al.} (GFitter Collaboration), Eur. Phys. J. C \textbf{72}, 2205 (2012).


\end{thebibliography}

